Cards Against AI: Predicting Humor in a Fill-in-the-blank Party Game

Humor is an inherently social phenomenon, with humorous utterances shaped by what is socially and culturally accepted. Understanding humor is an important NLP challenge, with many applications to human-computer interactions. In this work we explore humor in the context of Cards Against Humanity -- a party game where players complete fill-in-the-blank statements using cards that can be offensive or politically incorrect. We introduce a novel dataset of 300,000 online games of Cards Against Humanity, including 785K unique jokes, analyze it and provide insights. We trained machine learning models to predict the winning joke per game, achieving performance twice as good (20\%) as random, even without any user information. On the more difficult task of judging novel cards, we see the models' ability to generalize is moderate. Interestingly, we find that our models are primarily focused on punchline card, with the context having little impact. Analyzing feature importance, we observe that short, crude, juvenile punchlines tend to win.

==> 02formulation.tex <==
\section{Problem Formulation}

%i.e., predict which jokes are more likely to be picked as funniest by players. 

We define two tasks: 

\xhdr{Predicting a winner} Given a prompt and 10 punchlines, our goal is to predict the punchline most likely to be picked as funniest (Section \ref{task1}). 
%\dnote{this is really equivalent to saying pick the punchline. why complicate?}
%\donote{ Because we're trying to pick the joke, and the fact that players focus on the punchline is an artifact of the date/user behavior. Do you mean this about the second task? }\dnote{no. picking the best joke is equivalent to picking the best punchline, since the prompt is given per round}

\xhdr{Novel punchlines} We test whether our models can generalize to unseen punchlines (Section \ref{task2}). %In this task, the  %3) Exceptionally successful set-up and punchline combination jokes overall.


%we wish to pick the winning joke/combination per game. This is formulated as a ranking problem, wherein the inputs are the prompt and ten jokes, per game, and the prediction is which joke card was picked. Jokes may reoccur across different games with different (or the same) outcomes.   %Evaluation is performed using ranking at the round level - the top-1 accuracy.



==> old03.tex <==
\subsection{Methods}\label{methods1}
\dnote{this section has to be readable -- and with enough detail so people will actually understand what you used, what the features were, how you chose params}

The input data is structured with 1 row per prompt X punchline X game, and this input is used by all the models, which are then trained to predict if a given joke will be picked. For evaluation, predictions for all jokes are sorted in descending order according to the predicted score, then grouped at the round level for top-k accuracy evaluation. i.e., for top-1 accuracy, per each game the joke with the highest predicted probability of winning is kept, and is used for measuring accuracy. Results are aggregated over all games. This is effectively an admixture of a ranking and classification task.

The data was split into train and test subsets (80/20 split) at the level of games/rounds, with 195,708 rounds (1.9M rows, 746K unique jokes) for training, and the last 20\% (48,928 rounds, 367K unique jokes) as the test set. Target distribution was identical (10\%).

\subsubsection{Feature extraction}\label{Feature extraction 1}
Multiple feature extraction methods were used.  

1. Text features: ``Bag of words'' text features using the Catboost \cite{10.5555/3327757.3327770} library's inbuilt text encoder \footnote{\url{https://catboost.ai/en/docs/features/text-features}}.%bag of words were extracted from the lemmatized combined text column, as well as using % the Catboost library's inbuilt text encoder. %The "PairLogitPairwise" loss function was found to have the best performance [REF: \url{https://catboost.ai/en/docs/concepts/loss-functions-ranking#PairLogitPairwise}. We trained for 3K iterations.
% http://proceedings.mlr.press/v14/gulin11a.html - PairLogitPairwise loss paper, and latex for formula? 

2. Language model embeddings: A pretrained BERT \cite{DBLP:journals/corr/abs-2004-12765} based deep learning sentence level language model (``all-MiniLM-L12-v2'') from the Sentence-Transformers library \cite{reimers_sentence-bert_2019, DBLP:journals/corr/abs-2012-15828} was used for text embedding features.
Sentence level embeddings were extracted separately for each text column (prompt, punchline and joke/combined text).%, and distance/similarity features were extracted, as well as the raw embeddings. The final, “best” models used just the raw embeddings on the combined text column.
% We experimented with supervised finetuning of the model, but this did not work better than simply extracting the embeddings and training a supervised linear or random tree model atop the embeddings (these results were themselves inferior to the other models, and are not shown).
% We experimented with adapting the pretrained representation using masked language modelling and TSDAE tasks, on an unlabelled corpus of all the jokes in the data, but this did not yield notable improvements. 
%Embedding based modelling results are available: [ANONYMIZED PLACEHOLDER].%\url{https://colab.research.google.com/drive/1Ay-VYLAKGWvXhzug1SzCI8M7Yuwc618i  V2_SentenceBERT+sklearn-CAH.ipynb}.

3. A novel automated machine learning (autoML) framework - [redacted for anonymity]%SparkBeyond (See patent/US20170017900A1) \%
 was used to automatically extract and rank features from the data. Previous work has shown the benefit of autoML methods, in order to comprehensively and automatically find predictive signals in complex data \cite{9462159,Ofer2022.04.09.487727}. The system automatically extracts and ranks a wide range of features, including bag of words features, counts of words and characters, interactions between text columns, pretrained embeddings, and semantic features (such as Wordnet and Wikipedia concepts in the text). We note the autoML outperformed the other baseline modeling approaches used, even without using ranking models.

% 4. Finally, we made a combined model using the best features found using the autoML approach: it concatenated Catboost's text encoding features, the number of words and characters in the punchline, and the pretrained language model's embeddings of the joke.

\subsection{Models}\label{models1}
We tried the following models:
\begin{itemize}
    \item Catboost Ranking model, using the ``PairLogitPairwise'' loss described in \citet{pmlr-v14-gulin11a}) and default hyperparameters. The round identifier was used as the group for the model's ranking function. This model is aware of groups, and compares possible pairs of jokes within each group, where one is considered the winner and the other the loser and attempts to order them accordingly \footnote{\url{https://catboost.ai/en/docs/concepts/loss-functions-ranking#PairLogitPairwise}} . Inputs are groups of cards per round, with features from the Catboost inbuilt text encoder on the combined text input of each individual joke, and the round identifier. Internally, the model compares possible pairs of jokes, per round. 
    
    % \donote{https://catboost.ai/en/docs/concepts/loss-functions-ranking "Pairwise metrics use special labeled information — pairs of dataset objects where one object is considered the winner and the other is considered the loser. This information might be not exhaustive (not all possible pairs of objects are labeled in such a way). }.
    
    \item autoML + LightGBM classifier (default hyperparameters) - 300 top features selected by the autoML framework from the text columns, were used to train a LightGBM classification model \cite{10.5555/3294996.3295074} 
    
    \item Deep learning models - embeddings were extracted from the combined text column using the pretrained language models, as well as distance features (cosine and euclidean) between the punchline and prompt texts' embeddings. Different models (Logistic regression and a random forest from scikit-learn \cite{noauthor_scikit-learn_2012}, default hyperparameters) were trained using this input, as well as finetuning of the pretrained deep model itself. All results were inferior to the other ML approaches, and were discontinued \dnote{Maybe add "not shown"? We don't show these in the table 1}.
    \item Pairs popularity baseline - the prior win frequency of combinations (jokes) in the train set.
    \item Punchline Popularity baseline - the prior mean win frequency of the joke's constituent punchline in the train set (``Punchline Popularity''). Cases in the test data without training data coverage were imputed with the mean. We experimented with global smoothing and minimum occurrences, but found that this did not improve the baseline. Sorting by Punchline then by pairs, did not improve upon this baseline either (not shown).

    \item Combined model - A Catboost classifier model (default hyperparameters), that used multiple features: the Catboost inbuilt text encoder on the combined text input, embedding features on the combined text and the (autoML derived) number of words and characters in the punchline. This was also used for the second task \ref{task2}

Default hyperparameters were used for all final models. Model training time was a few minutes, on a private computer. Model training and combined feature extraction code is provided in the supplementary materials, and Github repository [redacted for anonymity].

\end{itemize}


\subsection{Results}
%\subsection{Predicting winning jokes}
\label{sec:Predicting winning jokes}

We predict the winning (''funniest``) joke (a combination of cards) in any given game and to rank the possible jokes per round accordingly. We note that unlike in traditional user-item ranking or “recommendation” tasks, we lack any user information.     
%We want to get a “funnyness” score for every joke, \%

We evaluated using ROC-AUC (area under the receiver operating characteristic curve) and top-1 accuracy (Acc@1), i.e., was the highest ranked card (out of 10) actually the winning card. A random baseline would thus get 10\% top-1 accuracy. We evaluated multiple models, including a ranking model that explicitly attempts to get the best pick per game using a pairwise loss, as well as a supervised classification model using features from the autoML framework. For the top-1 metric, the joke with the highest predicted score in each game was taken as the “top 1” pick, and evaluated accordingly. Results are shown below in Table \ref{Table 1 - Predicting winning games}).
We see that the combined and autoML approaches have the best results, but that their performance is equivalent to the punchline popularity baseline. We found that using only the punchline's prior win rate reached an average top 1 win rate of 20.5\% - outperforming random selection (10\%), but also effectively the same as that of the best models! 
In other words, most players cared only about the punchline, while prompts and context are mostly ignored!
%For the “popularity” baselines, we used all prompts, or pairs that appeared at least 1 time in the training data, and imputed the global average for missing values in the test data. \% “Popularity pairs” ranks jokes by the global prior expected win rate of a given joke (i.e prompt-punchline interactions). Popularity Baseline (Punchline) - ranks according to the prior average win-rate of just the punchline/white card. 


% \subsection{Table 1 - Predicting winning games}
% https://www.tablesgenerator.com/

\begin{table}
%\resizebox{\linewidth}{!}{%
%\parbox{
\begin{tabular}{lll}
Model & Acc@1 (\%) & AUC (\%) \\
\hline 
Catboost-Ranker & 18.7 & 61 \\
%("PairLogitPairwise")\% &  &  \\
AutoML Classifier & 20.2 & 64.3 \\
Punchline Popularity & 20.5 & 64.7 \\
Pairs Popularity & 15.6 & 55.8 \\
Combined & 20.2 & 64.3 \\
\end{tabular}
\caption{Predicting winning games \dnote{write the take-home message} \label{Table 1 - Predicting winning games}}
%}
%}
\end{table}
%% Popularity Baseline (Punchline) (game level) - top 2 acc: 35% , top 3 acc: 48%
%% at the game level, our ml model gets virtually the same score as the popularity baseline ; top 1 acc: 0.206 ,  top 2 acc: 0.356,  top 3 acc: 0.4864




%\subsubsection{Punchline popularity baseline}\label{subsubsection:Popularity baseline}

%Following insights gained from the autoML framework, surprisingly we found that the best models used only the white card/punchline texts, with no significant feature contributions from the interactions between the cards, or from the “context” (the prompt), as measured by feature importance and ablation testing (removing the prompt text as an input for the autoML feature extractor).
% Accordingly, we added a pseudo popularity baseline - the mean win ratio of a punchline (white card) in the training data (``Punchline Popularity''). Prompts in the test data without training data coverage were imputed with the mean. We experimented with global smoothing and minimum occurrences, but found that this did not improve the baseline. Adding the prior win rate of jokes (“Pairs Popularity” - Table \ref{Table 1 - Predicting winning games})), or the combination of sorting by punchline and joke prior, did not improve on this. Predicted results were ranked at the round level accordingly.

